Lexically-constrained Text Generation through Commonsense Knowledge Extraction and Injection

Conditional text generation has been a challenging task that is yet to see human-level performance from state-of-the-art models. In this work, we specifically focus on the Commongen benchmark, wherein the aim is to generate a plausible sentence for a given set of input concepts. Despite advances in other tasks, large pre-trained language models that are fine-tuned on this dataset often produce sentences that are syntactically correct but qualitatively deviate from a human understanding of common sense. Furthermore, generated sequences are unable to fulfill such lexical requirements as matching part-of-speech and full concept coverage. In this paper, we explore how commonsense knowledge graphs can enhance model performance, with respect to commonsense reasoning and lexically-constrained decoding. We propose strategies for enhancing the semantic correctness of the generated text, which we accomplish through: extracting commonsense relations from Conceptnet, injecting these relations into the Unified Language Model (UniLM) through attention mechanisms, and enforcing the aforementioned lexical requirements through output constraints. By performing several ablations, we find that commonsense injection enables the generation of sentences that are more aligned with human understanding, while remaining compliant with lexical requirements.

==> Tables/extraction_experiment.tex <==
\begin{table*}[t]
  \caption{Extraction results}
  \centering
  \begin{tabular}{lll}
    \toprule
    ~ & Avg num triples & Input concepts converge \\
    \midrule
    Multi-hop & 9.76 & 99.57 \\ 
    Knowledge selection & 7.04 & 99.57 \\ 
    Knowledge selection + Random sampling & 7.11 & 99.57 \\
    \bottomrule
  \end{tabular}
  \label{tab:extraction}
\end{table*}

% \begin{table}[ht]
%   \centering
%   \caption{Extraction results}
%   \resizebox{\columnwidth}{!}{
%   \begin{tabular}{|c|c|c|} \hline
%     ~ & Avg num triples & Input concepts converge \\ \hline
%     Multi-hop & 9.76 & 99.57 \\ \hline
%     Knowledge selection & 7.04 & 99.57 \\ \hline
%     Knowledge selection + Random sampling & 7.11 & 99.57  \\ \hline
% %    Unconstrained Random & 4.98 & 90.27 \\ \hline
%     \end{tabular}}
    
%     \label{tab:my_label}
% \end{table}
% %|m{2cm}| m{2cm} | m{2cm}| m{2cm} |


==> knowled_extraction_discussion.tex <==
\subsection{Knowledge Extraction}
We calculate the following two metrics for the evaluation of the proposed extraction methodologies:
\begin{itemize}
    \item Average number of relations: This gives us an idea of how many knowledge relations are extracted across all samples on average. 
    \item Concept Converge: The converge over input concepts will be the main metric for evaluating the extractions. This metric gives us an idea of how many proportion of input concepts are involved or missed in the extracted knowledge.
\end{itemize}
The multi-hop extraction obtains 9 knowledge relations on average across all input concept-sets. After knowledge selection (two models: length-based + Frequency-based knowledge selection and random subset knowledge selection), we reduce to around 7 relations on average. In terms of the converge score, our multi-hop extraction is able to cover 99.57 percentage of input concepts on average. It indicates that our extraction method is able to capture internal relations for almost all input concepts. The converge score will keep the same after constrained knowledge selections. 
